Worst-case time decremental connectivity and k-edge witness

We give a simple algorithm for decremental graph connectivity that handles edge deletions in worst-case time $O(k \log n)$ and connectivity queries in $O(\log k)$, where $k$ is the number of edges deleted so far, and uses worst-case space $O(m^2)$. We use this to give an algorithm for $k$-edge witness (``does the removal of a given set of $k$ edges disconnect two vertices $u,v$?'') with worst-case time $O(k^2 \log n)$ and space $O(k^2 n^2)$. For $k = o(\sqrt{n})$ these improve the worst-case $O(\sqrt{n})$ bound for deletion due to Eppstein et al. We also give a decremental connectivity algorithm using $O(n^2 \log n / \log \log n)$ space, whose time complexity depends on the toughness and independence number of the input graph. Finally, we show how to construct a distributed data structure for \kvw by giving a labeling scheme. This is the first data structure for \kvw that can efficiently distributed without just giving each vertex a copy of the whole structure. Its complexity depends on being able to construct a linear layout with good properties.

==> main.tex <==
\section{Introduction}
\label{sec:introduction}

In this paper we study decremental graph connectivity. In the edge deletion version of the problem, we are initially given an undirected graph $G$, and we can perform two operations: delete$(u,v)$, which deletes an edge $(u,v)$ from the current graph, and connected$(u,v)$ which returns whether vertices $u,v$ are connected. The vertex deletion version is the same, except that the delete operation is replaced with delete$(u)$, which deletes a vertex $u$ and all of its adjacent edges from the current graph.

The past decade has seen a good deal of effort in finding algorithms and data structures that efficiently support the above operations. However, the current best bounds known are amortized, expected, or even both. In 1992, Eppstein et al. \cite{EppGalIta-JACM-97} improved the worst-case bound of Frederickson \cite{808754} from $O(\sqrt{m})$ to $O(\sqrt{n})$ per update, and answering queries in constant time. This remains the best known worst-case bound for decremental connectivity on general graphs. Since then, there has been a number of improvements, in particular the work of Henzinger, King and Thorup \cite{320215,280036} who used randomization to obtain Las Vegas algorithms supporting updates in $O(\log^2 n)$ expected amortized time, and answering queries in $O(\log n / \log \log n)$ time. In 1998 Holm et al. \cite{502095} obtained a deterministic algorithm with $O(\log^2 n)$ amortized time for updates. However, none of these algorithms break the $O(\sqrt{n})$ worst-case barrier, and the amortized bounds are often taken over deleting all $m$ edges in a graph.

Our motivation for studying this problem comes from trying to efficiently represent cuts in a graph, and we are interested in the following problem, which we will call GRAPH CUT: given an undirected connected graph $G$, we want to answer queries ${\sf connected}(u,v,S)$, which returns `no' iff the set $S$ is a $uv$-cut in $G$' (in the edge cut version of the problem, $S$ is a set of edges and $S$ is a set of vertices in the vertex cut version).  We could answer queries using a fully-dynamic connectivity algorithm, by removing the set $S$ and testing connectivity, and then adding $S$ again to be ready for the next query, but the current best worst-case time would be $O(|S| \sqrt{n})$.

One interesting application is the `forbidden-set' routing problem for interdomain routing on the Internet \cite{}. Here, each autonomous system (AS) $u$ has a set $S$ of other ASes that it wishes to avoid in routing messages, perhaps because $u$ perceives these ASes to be unreliable, or because it is a competitor who may drop $u$'s traffic (in the edge version, $S$ would be a set of communication links that $u$ wishes to avoid). Furthermore, we expect that the sets $S(u)$ will be small, perhaps $O(\log n)$, but dynamically-changing.

In this paper we take a different approach to decremental connectivity that lets us improve on these worst-case bounds in special cases, in particular when the number of deletions is small, and when the graphs satisfy certain properties such as small cutwidth or path covering number. As far as we know, these are the first dynamic connectivity algorithms that make use of such graph properties, and that are optimised for small numbers of deletions.

%The main feature of our algorithms is that they have good worst-case time for both deletions and connectivity queries, although one artefact of our approach seems to be that the time for a deletion sometimes depends quadratically on the number of vertices or edges already deleted from the original graph. This occurs because we do not attempt any maintenance on the original graph after deletions, rather we just let it degrade, forcing future operations to incur a greater cost. Hence our bounds only represent an improvement for problems where the number of deletions is small. One approach to prevent such degredation is to repair the data structure at certain times, amortizing the cost of this operation over a sufficently large sequence of deletions. However, this would give amortized bounds (which we wanted to avoid), and we have also been unable to find an efficient way of repairing our data structures to give good amortized bounds. In light of the above, one might try to modify a well-known dynamic connectivity algorithm that has amortized bounds by allowing its structures to degrade, but we have been unable to do this.

%Our algorithms work by reducing the problem of maintaining decremental connectivity on some graph $G$ to maintaining fully dynamic connectivity (including insertions and deletions) on some auxiliary graph $H$, which is smaller and may have a simple structure, for example being a proper interval graph. We can then use known dynamic connectivity algorithms to maintain $H$, and answer connectivity queries on $G$ by translating them to queries on $H$.

%Finally, we show how to construct an efficient {\em distributed} data structure for the above problem, in the form of a labeling scheme: given a graph $G$, assign short labels $L$ to the vertices so that given only $L(u),L(v)$ and $L(S)=L(s_1),\ldots,L(s_k)$, we can efficiently decide if the set $S$ is a $uv$-cut of $G$. We are not aware of any current decremental connectivity algorithm that can be efficiently distributed in this way, without using large labels (i.e. assigning each vertex a copy of the whole data structure).

\subsection{Planar orthogonal range queries}
We make use of dynamic algorithms for planar orthogonal range queries to efficiently test for the existence of an edge in the auxiliary graph $H$ as follows. Given a linear layout $l$ of $G$, an edge $(u,v)$ of $G$ is a point $(l(u),l(v))$ in 2d space. Each vertex of the auxiliary graph $H$ represents a connected interval $[i,j]$ on the layout. Then two vertices $[a,b],[c,d] \in H$ are adjacent iff there exists an edge of $G$ with endpoints in $[a,b]$ and $[c,d]$ iff the box $[a,c] \times [b,d]$ is nonempty. If $G$ has $n$ vertices and $m$ edges, we can test for an edge in $H$ in worst-case time $O(\log n)$, and handle deletions and insertions of edges in worst-case time $O(\log n)$ \cite{644210}.

\section{Edge deletions}

Consider embedding the graph into a tree rather than a line. The tree still has the property that removing any edge disconnects it into two components, so this provides hope that we can efficiently maintain some sort of small auxiliary graph. In this section we give an decremental algorithm that handles the $k$th deletion in time $O(k \log n)$, and queries in time $O(k^2)$, regardless of the cutwidth or path number of the graph. Furthermore, the algorithm only requires $O(m)$ preprocessing time.

The algorithm is most similar to that of Henzinger and King \cite{320215}, with an exception -- instead of {\em maintaining} a spanning forest of $G$, we do not bother to patch up tree edges when they are removed. Instead, we keep track of the fragmented parts of the forest as edges are removed (using a dynamic connectivity algorithm) and use this information to efficiently answer the connectivity queries.

\begin{figure}
\small
\begin{verbatim}
initialise
  let T be a spanning tree of G
  number the vertices using a postorder traversal of T
  store the interval of T(v) for each vertex v
  insert edges of G into a range tree using the postorder numbering
  construct a graph H with a single vertex {[1..n]}

delete(u,v)
// assume that v > u, i.e. v is the parent of u
begin
 delete the edge (u,v) from G using the dynamic range tree [time=O(log n)]
 let h(u),h(v) be the intervals containing u,v
 if G has no edge between h(u),h(v) then [time=O(log n)]
 begin
   if h(u) != h(v) then
     delete the edge (h(u),h(v)) from H [time=O(1) using adjacency matrix]
   else
   begin
     let h=h(u)=h(v)
     // split the vertex h
     let [i,j] = T(u), the subtree rooted at u

     let [a,b] be the interval of H containing i
     if (a < i) then
       delete [a,b] from H
       insert [a,i-1],[i,b] into H
       for each neighbour [x,y] of [a,b] in H
         if G has an edge ([x,y],[a,i-1]) then add an edge ([x,y],[a,i-1]) to H
         if G has an edge ([x,y],[i,b]) then add an edge ([x,y],[a,i-1]) to H

     let [c,d] be the interval of H containing j
     if (d > j) then
       delete [c,d] from H
       insert [c,j],[j+1,d] into H
       for each neighbour [x,y] of [c,d] in H
         if G has an edge([x,y],[a,i-1]) then add an edge ([x,y],[a,i-1]) to H
         if G has an edge([x,y],[i,b]) then add an edge ([x,y],[a,i-1]) to H

   end
 end
end

connected(u,v)
  find h(u), h(v) [time=O(log |H|)]
  do a dfs on H [time=O(|H|^2)]
\end{verbatim}
\label{fig:algorithm1}
\caption{The tree embedding algorithm}
\end{figure}

The algorithm maintains a graph $H$ whose vertices are connected subtrees of $T$, with an edge between two subtrees $h_1,h_2$ if there is a nontree edge of $G$ between a pair of vertices $u \in h_1, v \in h_2$. Deleting a tree edge $(u,v)$ where $v$ is the parent of $u$ and $T(u)=[i,j]$ is done by splicing out the interval $[i,j]$ from the set of intervals covering it, which results in splitting a vertex of $H$. The above implementation stores $H$ in adjacency matrix form so that edge updates are $O(1)$.

Each tree edge deleted increases the number of vertices of $H$ by at most 2, so after $k$ deletions $H$ has $O(k)$ vertices. The $k$th deletion takes worst-case time $O(k \log n)$, and connectivity queries are answered in worst-case time $O(k^2)$. Alternatively we could use the algorithm of Eppstein to maintain $H$ (where each edge deletion or insertion takes worst-case time $O(\sqrt{|H|})$), so that the $k$th deletion takes time $O(k^{3/2} + k \log n)$ and connectivity queries are answered in time $O(\log k)$.

